Data Integrity Error Localization in Networked Systems with Missing Data

Most recent network failure diagnosis systems focused on data center networks where complex measurement systems can be deployed to derive routing information and ensure network coverage in order to achieve accurate and fast fault localization. In this paper, we target wide-area networks that support data-intensive distributed applications. We first present a new multi-output prediction model that directly maps the application level observations to localize the system component failures. In reality, this application-centric approach may face the missing data challenge as some input (feature) data to the inference models may be missing due to incomplete or lost measurements in wide area networks. We show that the presented prediction model naturally allows the {\it multivariate} imputation to recover the missing data. We evaluate multiple imputation algorithms and show that the prediction performance can be improved significantly in a large-scale network. As far as we know, this is the first study on the missing data issue and applying imputation techniques in network failure localization.

==> emulation.tex <==
We use the NSF ExoGENI cloud testbed~\cite{ExoGENI:web} to create a virtual network for our training data generation. We specifically emulate aspects of the Open Science Grid (OSG)~\cite{OSG:web} data federation network that is highly utilized to distribute data for high throughput scientific computing. Pegasus, a popular WMS to coordinate the data transfer and compute job submission in such an environment, has recently added end-to-end flow level integrity error checking capability~\cite{swip:pearc:2019}.    

In order to simulate different types of sources of integrity errors, we added a new utility in Chaos Jungle~\cite{swip:pearc:2019,chaosjungle:web}, which can corrupt arbitrary file(s) in nodes in addition to packets out of network interfaces according to a given probability. This tool gives us the capability to inject controlled errors into any network elements using several integrity threat models~\cite{threat-model}.

One of our main design objectives is to automate the experiment creation, configuration, and data collection at any given scale. This not only guarantees repeatable experiments at different scales, but also makes data manipulation for ML model training for RCA much more efficient.    

\subsection{Network creation and configuration}
An arbitrary topology can be created on ExoGENI with nodes in the form of virtual machines (VM) running customized images. In our experimental topology, we use a set of end hosts to emulate the OSG data sources and sinks, a virtual network consisting of core routers emulating the backbone network service providers (Internet2, ESNet, etc.) and access routers emulating the access network service providers (regional research and education networks and campus networks). All nodes are connected with virtual layer-2 links with certain throughput guarantee as the private data plane. An extra management plane interface is also available on every node, which provides remote access. The end hosts run an Ubuntu image with our Chaos Jungle fault injection tools. The routers run an Ubuntu image with the Zebra software router and our Chaos Jungle fault injection tools.

ExoGENI provides an API to launch any given experimental topology. On a successful execution, our experimental topology will be up and running with routing configured and network reachability established among all end hosts by leveraging the postboot template scripting capability provided by ExoGENI. Specifically, at the virtual node booting, following steps are automatically executed: (1) detecting all the interfaces and their IP addresses, and all the neighboring nodes and the links; (2) creating the configuration files for Zebra and OSPF daemons and starting the routing control plane at the router nodes; (3) adding the default routes at the end hosts.    

\subsection{Data transfer and fault injection}
For every experiment, we attach a controller node that can reach all the nodes in the topology via the management plane interface. The controller is provided a Postboot script that automatically learns the experimental topology, creates a list of end hosts, routers, and links, and populates the end hosts with a set of files for the data transfer.

A user can log into the controller node, modify the experimental configuration files that define the data origin and sink nodes, the list of nodes to introduce storage integrity error, the list of network link interfaces to be disrupted by the Chaos Jungle tool, and the fault injection probability.

Then the experiment software can be started to inject the fault, transfer the data files from the origins, check the integrity at the sinks, and collect the data. This sequence is repeated for every fault specified in the configuration file.

\subsection{Data collection and analysis}
At the last step, all the raw data will be processed and stored in final result database files with predefined feature columns. Each database entry represents one data transfer with features of file name, file size, origin, sink, access router, integrity error or not, etc. However, the forwarding path is unknown as it is controlled by the routing control plane process. The final result is exported to a Jupyter notebook environment where machine learning based data analysis is performed.

The experimental topology used in this paper is shown in Fig.~\ref{fig:topology}, the screenshot from the ExoGENI GUI.
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{./figure/ChaosJungle}
\end{center}
\vspace{-0.05in}
\caption{Network Emulation and Integrity Error Injection in ExoGENI}
\vspace{-0.05in}
\label{fig:topology}
\end{figure}
%\begin{figure}[!ht]
%\begin{center}
%\includegraphics[width=0.48\textwidth]{./figure/experiment-large}
%\end{center}
%\caption{Experimental Topology}
%\label{fig:topology}
%\end{figure}




==> reference.tex <==

"prior distribution -> posterior distribution" : "1.  reduce overfitting from small data set by bringing in prior distribution and knowledge; 2. scalability of ML; 3. the ability to express the uncertainty of predictions is one of the most important capabilities of Bayesian learning".

"Deep exponential families (e.g., deep latent Gaussian models)", "Gaussian process models (e.g., regression / classification)", "reinforcement learning (Bayesian Reinforcement Learning) "

"For classification problems we wish to construct models
that are able to accurately to predict categorical output. For a machine learning classification algorithm that produces probabilistic output,
one approach is to model the probability mass function of the output given the input"~\cite{RW06:GP}.

"Consider a case where we are given inputs x1, . . . , xn ? $X_i$ with corresponding outputs y1, . . . , yn ? {?1, 1}. In this work we will assume that X ? Rd, although in reality the inputs could have categorical components. Here yi is referred to as the class or output corresponding to the input xi, and D = {(x1, y1), . . . , (xn, yn)} is called the training dataset since it is the data that will be used to train a classifier."

Two common choices of prior distribution: the cumulative distribution functions of the standard normal distribution and the standard logistic distribution. In the context of Gaussian process classification they are known as the cumulative Gaussian likelihood function and the logistic likelihood function.

~\cite{gp:on:2018}, As was pointed out, the examined fault localization scheme consists of two phases. The first phase is activated upon the detection of a failure and consists of correlating the affected and unaffected lightpaths. For the path correlation phase, the GBC heuristic [13] is used. The second phase is activated only if the GBC heuristic reports that multiple links are suspected of causing the failure. This phase consists of computing a failure probability for each suspect link. The failure probability is computed by a GP classifier trained on a set that describes past failure incidents. 

the MTBF of each link in the network follows the Weibull distribution. we count (1) the total number of failures in the network $C(n)$ and (2) the number of failures $c_{j}$ associated with each link $e_j$ in the network, up to the last known failure incident $i$. Then, by dividing $C_j(n)$ by $C(n)$ for each incident $i$, we can compute the failure rate of each link $j$ at each time point.

Such historical information can then be utilized by a probabilistic model to find the likelihood that a link $e_j$ is the failed link upon incident i. The class of GPs is one of the most widely used families of stochastic processes for modeling dependent data observed over time. Thus, GPs are useful for sequential data, such as time-series and tracking applications, and can be used in particular for active data selection in such systems [16]. GPs constitute one of the most important Bayesian ML approaches and are based on a particularly effective method for placing a prior distribution over the space of regression functions. They have a small number of tunable parameters, can be trained on relatively small training sets, and allow us to capture nonlinear and skewed artifacts, thus exhibiting significant robustness to outliers and the ability to handle sparse data without becoming prone to overtraining. Compared to another popular form of discriminative kernel machines, i.e., the support vector machine (SVM) [17], GPs possess several advantages, with the most significant being that the GP model produces an output with a clear probabilistic interpretation, providing a measure of uncertainty for the obtained predictions, unlike SVMs, which merely provide point predictions [18].
------------------------

~\cite{Boulle:2019aa}
Boullé, M., Charnay, C.  Lachiche, N. A scalable robust and automatic propositionalization approach for Bayesian classification of large mixed numerical and categorical data. Mach Learn 108, 229,266 (2019).

We introduce a propositionalization approach dedicated to a robust Bayesian classifier. It efficiently samples a given number of features in the language bias, following a distribution over the complex aggregates.  
using aggregation functions such as minimum, maximum or average in order to deal with both the numerical attributes and the one-to-many relationship, whether existing relational data mining systems can be used on large mixed, numerical and categorical, data, and in particular whether increasing the expressivity by using complex features increases overfitting too and whether their runtimes and memory consumption are acceptable.
Propositionalization transforms the relational data into an attribute-value dataset in order to use attribute-value learners the data scientists may be familiar with. 
? Count(Table)?Num count of records in a table,
? Mode(Table, CatFeat)?Cat most frequent value of a categorical feature in a table,
? CountDistinct(Table, CatFeat)?Num number of distinct values,
? Mean(Table, NumFeat)?Num mean value of a numerical feature in a table, ? Median(Table, NumFeat)?Num median value,
? Min(Table, NumFeat)?Num min value,
? Max(Table, NumFeat)?Num max value,
? StdDev(Table, NumFeat)?Num standard deviation, ? Sum(Table, NumFeat)?Num sum of values.

Our proposition for solving these problems is the introduction of an evaluation criterion of the constructed features according to a Bayesian approach in order to penalize complex features. This is called regularization. In order to implement this evaluation criterion, we propose a prior distribution on the space of all features and an efficient sampling algorithm of the space of features according to their prior distribution. Our approach builds upon the MODL supervised preprocessing methods (Boullé 2005, 2006). These methods consists in partitioning either a numerical features into intervals or a cate- gorical feature into groups of values, through a piecewise constant class conditional density estimation.

Boullé (2006) for supervised discretization and Boullé (2005) for supervised value grouping.
------------------


 the intermittent and random nature of 
the distributed nature and stringent resources of WSNs render it hard for a network operator to completely monitor the system?s working status.
On the other hand, the interactions within the WSN and the causal dependencies between root causes and symptoms are usually unknown.
As a result, silent failures remain undetected.

It belongs to the broader {\it'gray failures'}, {\it'silent failures'}, {\it'probabilistic failures'}  in contrast to the {\it fail-stop} failures where

damages: service disruption, waste of time in retrying, data corruption leading to wrong results and decisions. 
  
Error tolerance, redundancy, overhead in resource and latency

end-too-end check at the file or block level, overhead in computing and latency.

localization has been ignored

error family and error locations at different granularity 


---------------------------------------------------------

The root causes of the failure may come from the network devices or the storage or compute servers at the edge clusters. The network devices and cluster servers demonstrate very different failure characteristics and are managed by different system administrative groups. More specifically, their probabilistic distributions are in different magnitude ranges.     

In this paper, we designed a two-step machine learning classification approach that combine a decision tree model to identify a subset of possible failure root causes and a statistical learning model to 
compute the probabilistic likelihood of these causes. 



In this paper, we first cast the WMS integrity error diagnosis as a networked system Root Cause Analysis (RCA) problem, where limited network system information is available for end-to-end data transfers (Section~\ref{sec:integrity}). Our main hypothesis is that the mapping between the end host level flow statistics and the possible network component failures can be learned and inferred from sufficiently large amount of labeled training data. In order to obtain sufficient amount of training data and make repeatable experiments more efficient, we created an experimental system in a Cloud testbed that can automatically create a large-scale OSPF-enabled virtual network system, initiate data transfers between end hosts, and inject arbitrary integrity errors into the virtual router interfaces and end hosts (Section~\ref{sec:emulation}). We then studied several variants from three different families of multi-class classification models, Bayesian inference, SVM, and Decision Tree, and validated their accuracy performance using a Top-$k$ accuracy metric (Section~\ref{sec:ml}). With the data collected from the emulation, we evaluate their accuracy in Section~\ref{sec:evaluation}. We specifically studied the impact of available data transfer data in terms of end host pair coverage. We conclude the paper with our future research plan in Section~\ref{sec:future}.


It has been recently recognized that existing protection mechanisms commonly implemented in Internet and distributed systems such as TCP checksums and redundant coding in storage systems are not sufficient to handle silent {\it gray failures}, which often lead to wide spread system slowdown, application malfunction, and corrupted data. As a result, advanced distributed systems started to add extra end-to-end data integrity checks to catch these failures early on in order to reduce application failures and blind retries~\cite{swip:pearc:2019}. 

However, identifying the root causes of these gray failures remains a largely unsolved problem due to the challenges presented in Section~\ref{sec:introduction}: 
incomplete network state information, intermittent probabilistic nature of gray failures, and complexity in diagnosing complex networks in a scalable fashion.  

A network system can be modeled as a graph with a set of nodes connected by links via interfaces. The nodes in the network consist of end hosts (that generate and receive data) and networking devices (routers or switches). Due to scalability or privacy constraints, deploying monitoring capabilities at every point of the targeted large-scale network is not possible. Therefore, the problem can be concisely modeled as a bipartite mapping graph between the path level flows and its network components as shown in Fig.~\ref{fig:bipartite}. What makes the problem extremely difficult is that the mapping relationships in the bipartite graph are unknown. We further observe that one component failure (e.g., $L_j$) will cause multiple paths erroneous while one flow error (e.g., $F_i$) may be caused by multiple component failures. And because the component gray failure probability is normally low ($10^{-3} - 10^{-6}$), it would require large number of file transfers to catch a few number of corrupted files. Our ultimate goal is to localize the possible root causes in node or link errors by inference from the observed flow level abnormalities only at the end hosts, which can be translated to learning the mappings in such a graph.

\begin{wrapfigure}{ht}{0.25\textwidth}
  \begin{center}
    \includegraphics[width=0.25\textwidth]{./figure/RCABipartite}
  \end{center}
  \vspace{-5pt}
\caption{RCA Bipartite Graph}
\vspace{-5pt}
\label{fig:bipartite}
\end{wrapfigure}

The majority of recent work assume flow information between any pair of nodes in the network is available because they focus on data center networks that they have full ownership and modern routers allow originating and receiving probing data. This is very important because, as shown in~\cite{netbouncer:nsdi18}, there exists a minimal set of source-destination pairs to guarantee successful pinpointing of link errors in the network. Some of the work further assume they even know the routes for every flow, i.e., the mapping represented in Fig.~\ref{fig:bipartite}. However, both assumptions do not hold for our targeted multi-domain network environment due to obvious administrative constraints and the fact that, in the Internet scale network, traffic routing and forwarding are largely dynamically decided by the control plane software like OSPF and BGP subject to frequent topology and policy changes. 

We therefore made more restrictive but more realistic assumptions in this study in that (1) only the data file transfer information including integrity error states can be obtained at the end hosts from application layer; (2) only the physical nodes (domains) and their interfaces are known to us, but the network topology and traffic routing are unknown. 

In a large network, collecting the passive monitoring data from all node pairs may not scale well. Therefore, injecting probe packets between the designated node pairs periodically is adapted by several existing RCA systems. In practice, due to the probabilistic nature of the grey failures, controlled fault injection is an efficient way to generate training data within a reasonable time frame.

Directly accessing the production system to instrument the analysis with either active probing or fault injection is not realistic in most cases, especially in a multi-domain system where no one owns the entire infrastructure like in the data center networks. We believe emulation with realistic scales is a viable choice, given advanced Cloud testbeds are available.


